Unitho: A Unified Multi-Task Framework for Computational Lithography

Reliable, generalizable data foundations are critical for enabling large-scale models in computational lithography. However, essential tasks-mask generation, rule violation detection, and layout optimization-are often handled in isolation, hindered by scarce datasets and limited modeling approaches. To address these challenges, we introduce Unitho, a unified multi-task large vision model built upon the Transformer architecture. Trained on a large-scale industrial lithography simulation dataset with hundreds of thousands of cases, Unitho supports end-to-end mask generation, lithography simulation, and rule violation detection. By enabling agile and high-fidelity lithography simulation, Unitho further facilitates the construction of robust data foundations for intelligent EDA. Experimental results validate its effectiveness and generalizability, with performance substantially surpassing academic baselines.

==> figs/union-comp.tex <==
\begin{tikzpicture}[scale=0.45]
% 定义颜色
\definecolor{darkyellow}{RGB}{31, 119, 180} 
\definecolor{lightyellow}{RGB}{174, 199, 232} 
\definecolor{darkred}{RGB}{148, 103, 189}
\definecolor{lightpink}{RGB}{197, 176, 213}

% 定义数据点的标签和角度
\def\labels{{"Recall", "Precision", "$F_1$", "\#FA($\times 1$K)", "AP"}}
\def\numaxes{5}
% 定义两组数据
\def\datared{{79.85, 81.44, 80.64, 7.704, 82.24}}
\def\datablue{{68.12, 73.43, 70.67, 10.438, 73.92}}

% 左侧雷达图 - Detection-Only
\begin{scope}[xshift=-120pt]
    % 绘制同心圆网格
    \foreach \r in {20,40,60,80} {
        \draw[gray, dashed, very thin] (0,0) circle (\r pt);
    }
    
    % 绘制坐标轴
    \foreach \i in {0,...,4} {
        \pgfmathsetmacro{\angle}{90-\i*360/\numaxes}
        \draw[gray, thin] (0,0) -- (\angle:80pt);
        % 添加标签
        \pgfmathsetmacro{\labeltext}{\labels[\i]}
        %\node at (\angle:95pt) {\labeltext};
        \node[font=\footnotesize] at (\angle:95pt) {\labeltext};
    }
    
    % 绘制红色数据填充区域
    \coordinate (red0) at ({90-0*360/\numaxes}:{\datared[0]*0.8pt});
    \foreach \i [remember=\i as \lasti (initially 0)] in {1,...,4} {
        \pgfmathsetmacro{\angle}{90-\i*360/\numaxes}
        \coordinate (red\i) at (\angle:{\datared[\i]*0.8pt});
    }
    \fill[lightpink, opacity=0.3] (red0) -- (red1) -- (red2) -- (red3) -- (red4) -- cycle;
    
    % 绘制红色数据线
    \foreach \i [remember=\i as \lasti (initially 0)] in {1,...,4} {
        \draw[darkred, thick] (red\lasti) -- (red\i);
    }
    \draw[darkred, thick] (red4) -- (red0); % 闭合路径
    
    % 添加数据点
    \foreach \i in {0,...,4} {
        \pgfmathsetmacro{\angle}{90-\i*360/\numaxes}
        \fill[darkred] (\angle:{\datared[\i]*0.8pt}) circle (1.5pt);
    }
    
    % 添加数值标签
    \foreach \i in {0,...,4} {
        \pgfmathsetmacro{\angle}{90-\i*360/\numaxes}
        \pgfmathsetmacro{\redval}{\datared[\i]}
        \node[darkred, font=\scriptsize] at (\angle:{\datared[\i]*0.8pt+8pt}) {\redval};
    }
    
    % 添加刻度标签
    \foreach \r in {20,40,60,80} {
        \node[font=\tiny, gray] at (0:\r pt+3pt) {\pgfmathparse{\r/0.8}\pgfmathprintnumber{\pgfmathresult}};
    }
    
    % 标题
    \draw[darkred, very thick, line cap=round] (-115pt, -115pt) -- (-100pt, -115pt);
    \node[font=\small, black] at (0, -115pt) {\textbf{Sandalone Detection}};
\end{scope}

% 右侧雷达图 - Union
\begin{scope}[xshift=120pt]
    % 绘制同心圆网格
    \foreach \r in {20,40,60,80} {
        \draw[gray, dashed, very thin] (0,0) circle (\r pt);
    }
    
    % 绘制坐标轴
    \foreach \i in {0,...,4} {
        \pgfmathsetmacro{\angle}{90-\i*360/\numaxes}
        \draw[gray, thin] (0,0) -- (\angle:80pt);
        % 添加标签
        \pgfmathsetmacro{\labeltext}{\labels[\i]}
        %\node at (\angle:95pt) {\labeltext};
        \node[font=\footnotesize] at (\angle:95pt) {\labeltext};
    }
    
    % 绘制蓝色数据填充区域
    \coordinate (blue0) at ({90-0*360/\numaxes}:{\datablue[0]*0.8pt});
    \foreach \i [remember=\i as \lasti (initially 0)] in {1,...,4} {
        \pgfmathsetmacro{\angle}{90-\i*360/\numaxes}
        \coordinate (blue\i) at (\angle:{\datablue[\i]*0.8pt});
    }
    \fill[lightyellow, opacity=0.3] (blue0) -- (blue1) -- (blue2) -- (blue3) -- (blue4) -- cycle;
    
    % 绘制蓝色数据线
    \foreach \i [remember=\i as \lasti (initially 0)] in {1,...,4} {
        \draw[darkyellow, thick] (blue\lasti) -- (blue\i);
    }
    \draw[darkyellow, thick] (blue4) -- (blue0); % 闭合路径
    
    % 添加数据点
    \foreach \i in {0,...,4} {
        \pgfmathsetmacro{\angle}{90-\i*360/\numaxes}
        \fill[darkyellow] (\angle:{\datablue[\i]*0.8pt}) circle (1.5pt);
    }
    
    % 添加数值标签
    \foreach \i in {0,...,4} {
        \pgfmathsetmacro{\angle}{90-\i*360/\numaxes}
        \pgfmathsetmacro{\blueval}{\datablue[\i]}
        \node[darkyellow, font=\scriptsize] at (\angle:{\datablue[\i]*0.8pt+8pt}) {\blueval};
    }
    
    % 添加刻度标签
    \foreach \r in {20,40,60,80} {
        \node[font=\tiny, gray] at (0:\r pt+3pt) {\pgfmathparse{\r/0.8}\pgfmathprintnumber{\pgfmathresult}};
    }
    
    % 标题
    \draw[darkyellow, very thick, line cap=round] (-40pt, -115pt) -- (-25pt, -115pt);
    \node[font=\small, black] at (5pt, -115pt) {\textbf{Union}};
\end{scope}

\end{tikzpicture}
